Depth Completion via Deep Basis Fitting

In this paper we consider the task of image-guided depth completion where our system must infer the depth at every pixel of an input image based on the image content and a sparse set of depth measurements. We propose a novel approach that builds upon the strengths of modern deep learning techniques and classical optimization algorithms and significantly improves performance. The proposed method replaces the final $1\times 1$ convolutional layer employed in most depth completion networks with a least squares fitting module which computes weights by fitting the implicit depth bases to the given sparse depth measurements. In addition, we show how our proposed method can be naturally extended to a multi-scale formulation for improved self-supervised training. We demonstrate through extensive experiments on various datasets that our approach achieves consistent improvements over state-of-the-art baseline methods with small computational overhead.

==> acknowledgment.tex <==
\section*{ACKNOWLEDGMENT}

The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.

==> bibliography.tex <==
\begin{thebibliography}{99}

\bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
\bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
\bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
\bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
\bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
\bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
\bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
\bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
\bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
\bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
\bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
\bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
\bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
\bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
\bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
\bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
\bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
\bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
\bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
\bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 

\end{thebibliography}


==> macro.tex <==
\newcommand{\LSF}{least squares fitting}

==> s70_rebuttal.tex <==
\section{Response}

We thank all the reviewers for their valuable feedback. 
We address each reviewer's comments in the following sections. 
We provide supporting experiments in both the main paper and the supplementary material.

\input{s71_reviewer1.tex}
\input{s72_reviewer3.tex}
\input{s73_reviewer4.tex}

\subsection{Changes Made}
We added extra experiments against other methods (PnP\cite{wang2018pnp}, CSPN\cite{Cheng2018DepthEV}) to the main paper and evaluation on another baseline (FusionNet\cite{Gansbeke2019SparseAN}) to the supplementary material as requested. 
We also add more ablation study addressing all concerns raised by the reviewers.
We found and fixed a bug in evaluating NYU-V2 dataset and all related numbers are updated.

==> s71_reviewer1.tex <==
\subsection{To Reviwer \#1}

\noindent \textbf{Comparison with other Methods.}
We add comparison against PnP \cite{wang2018pnp}, which is the most similar work to ours in that it can be added to an existing network, but requires no re-training.
We also compare with CSPN \cite{Cheng2018DepthEV}.
We are unable to reproduce their results with our baseline network, thus we take the numbers from their paper and KITTI benchmark directly.
Please see \textbf{Section 4.2 Results} in the main paper.

We then attach our LSF module to another depth completion network FusionNet \cite{Gansbeke2019SparseAN} which uses an ERFNet\cite{Romera2018ERFNetER} backbone.
Please see \textbf{Section 7.1 FusionNet} in the supplementary material.

\vspace{\baselineskip}
\noindent \textbf{Number of Iterations.}
We empirically found that the least squares fitting usually converges within 2 iterations.
Please see \textbf{Section 6.5 Number of Iterations} in the supplementary material.

==> s72_reviewer3.tex <==
\subsection{To Reviwer \#3}

\noindent \textbf{Weak Baseline.}
The decoder is symmetric to the ResNet18 encoder, and thus has channel widths (256, 128, 64, 64).
The (4, 8, 16, 32) multi-scale basis are produced by extra convolutions on top of the decoder output at each scale (not the width of the decoder).
As such, the baseline network with ResNet18 has around 15M parameters which is not small.
Similar networks have been used in other state-of-the-art depth prediction work \cite{Godard2018DiggingIS}.
For NYU-V2 dataset, we only use the 1449 densely labelled image depth pairs for training and validation, this could be one of the reasons that our rgb baseline is weak on this particular dataset.

DORN\cite{Fu2018DeepOR}, on the other hand, uses ResNet101 (more than 51M parameters), is trained jointly on the full KITTI, Make3D and NYU-V2 datasets for more than 3M iterations.
Due to the large amount of experiments we have to run, it is impossible for us to adopt such a heavy network and training strategy.

% Since our module can be attached to most depth prediction networks, we made the choice to conduct controlled experiments rather than push for numbers.
% Specifically, we design our experiments such that everything (all random seeds, network parameters, initialization, learning rate, data augmentation, \etc) is the same except for the final convolution layer. 
% Note that we didn't introduce a module that adds extra parameters to the baseline, 
% on the contrary, our module has even fewer parameters (albeit a small amount).
% Therefore, we are confident to claim that any improvements upon the baseline is due to our proposed method, not by extra parameters or other unexplainable factors.

\vspace{\baselineskip}
\noindent \textbf{Comparison with other Methods.}
This same point is also raised by reviewer \#1. 
Please see the same section in our reply to reviewer \#1.

\vspace{\baselineskip}
\noindent \textbf{Multi-scale Bases.}
Predicting depth at multiple scales is necessary to overcome the gradient locality problem in self-supervised training \cite{Zhou2017UnsupervisedLO}.
The reason we use multi-scale formulation is that it outperforms singles-scale bases even in supervised training where only the full resolution depth map is needed.
Please see \textbf{Section 6.3 Mutli-scale Bases} in the supplementary material.

\vspace{\baselineskip}
\noindent \textbf{Nonlinear Activation.}
Although some works simply use a ReLU activation to produce final depth, 
the (inverse) sigmoid function is another popular choice for depth prediction \cite{Godard2018DiggingIS, Zhou2017UnsupervisedLO, Wang2017LearningDF}.
We chose it for the following reasons. 
1) we would like to predict inverse depth (disparity) for self-supervised training,
and sigmoid activation is the standard choice.
2) ReLU activation will cause some depth values to be 0.
This can be fixed by adding a small value to the depth, but using a sigmoid function has no such issue.

Nevertheless, our proposed method would still work with a ReLU activation, 
except that there's no need for a nonlinear fitting. 
We show this in experiments using FusionNet \cite{Gansbeke2019SparseAN} as a baseline, where the final activation is simply ReLU.
Note that FusionNet does not have multi-scale prediction, thus we use a single scale basis.
Please see \textbf{Section 7.1 FusionNet} in the supplementary material.

\vspace{\baselineskip}
\noindent \textbf{Underdetermined System.}
We conduct experiments with fewer depth samples than the size of the bases to create an underdetermined system for our module.
With the regularization parameter, our module will still produce a solution, but with degraded results. 
Please see \textbf{Section 6.4 Underdetermined System} in the supplementary material.

\vspace{\baselineskip}
\noindent \textbf{Kernel Size.}
It is possible to use a bigger kernel size for the final convolution, e.g. $3\times3$, rather than the $1\times 1$ filter we used across the paper. 
This effectively increase the dimension of the bases by 9, and one could easily achieve this by re-arranging the penultimate feature maps so that the final kernel size is still $1\times1$. 
For this reason, we only work with $1\times 1$ kernel as it is the most general case.

==> s73_reviewer4.tex <==
\subsection{To Reviewer \#4}

\noindent \textbf{Outlier Mask.} 
The outlier mask is generated from the robust loss function (Huber loss).
When the standardized error between a sparse depth sample and the fitting result is greater than 1, 
it is considered an outlier.
This mask is not used explicitly during training, only for visualization.
